Learning Stabilizing Latent Feedback Controllers via Multi-Step Backward Losses

Can learned latent dynamics models support the design of feedback controllers that provably stabilize the original system? For linear time-invariant systems, we show that learning linear autoencoders and latent dynamics with multi-step prediction-reconstruction losses $\unicode{x2014}$ which we term "backward losses" as they encourage latent trajectories to reconstruct full state trajectories $\unicode{x2014}$ provably recovers the structure needed for stabilization. Specifically, a sufficiently long reconstruction horizon ensures that a minimum ${H}_\infty$-norm controller designed using the learned latent model stabilizes the original system through output-feedback via the corresponding encoder, provided the latent dimension is large enough to capture all non-stable modes of the underlying system. We also show why both reconstruction and a multi-step horizon are essential: forward prediction losses that require only low prediction error along latent trajectories admit global loss minimizers that discard unstable modes regardless of horizon length, while single-step reconstruction losses can yield latent models whose stabilizing controllers fail to stabilize the original system. Finally, experiments on a non-linear flexible-arm system illustrate the practical implications of our results for learning non-linear autoencoders and latent dynamics.

==> tables/linear_conjugacy.tex <==
$\mathcal{L}_{\mathrm{bwd}}^{(T)}$ & $R_{\mathrm{orth}}$ & pop. & $1$ & $0.034$ & $2.2\cdot 10^{-4}$ & $5.5\cdot 10^{-5}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & $100$ & $1$ & $0.057$ & $2.3\cdot 10^{-4}$ & $6.8\cdot 10^{-5}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & $500$ & $1$ & $0.039$ & $2.3\cdot 10^{-4}$ & $6.8\cdot 10^{-5}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & $1000$ & $1$ & $0.035$ & $2.2\cdot 10^{-4}$ & $6.2\cdot 10^{-5}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & $R_{\mathrm{vr}}$, $\mathsf{N}(0,I)$ & pop. & $0.99$ & $0.034$ & $2.2\cdot 10^{-4}$ & $8.8\cdot 10^{-5}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & $R_{\mathrm{sr}}$, $\mathsf{N}(0,I)$ & pop. & $0.051$ & $0.036$ & $2.3\cdot 10^{-4}$ & $1.1\cdot 10^{-4}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.75 \\
 & $R_{\mathrm{vr}}$, traj. & pop. & $1.5\cdot 10^{-3}$ & $2$ & $3.9\cdot 10^{-3}$ & $1.8\cdot 10^{-3}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & $100$ & $7.0\cdot 10^{-4}$ & $1.6$ & $7.5\cdot 10^{-3}$ & $2.3\cdot 10^{-3}$ & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.57 & 0.40 \\
 &  & $500$ & $6.2\cdot 10^{-4}$ & $2.8$ & $2.3\cdot 10^{-3}$ & $2.8\cdot 10^{-3}$ & 0.80 & 0.80 & 0.55 & 0.40 & 0.40 & 0.28 & 0.20 \\
 &  & $1000$ & $4.1\cdot 10^{-4}$ & $2.1$ & $1.7\cdot 10^{-3}$ & $1.3\cdot 10^{-3}$ & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.75 & 0.55 \\
 & $R_{\mathrm{sr}}$, traj. & pop. & $0.028$ & $0.064$ & $3.4\cdot 10^{-4}$ & $4.5\cdot 10^{-4}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.75 \\
 &  & $100$ & $0.053$ & $0.17$ & $7.1\cdot 10^{-4}$ & $1.8\cdot 10^{-4}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.65 \\
 &  & $500$ & $0.049$ & $0.11$ & $4.3\cdot 10^{-4}$ & $1.0\cdot 10^{-3}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.70 \\
 &  & $1000$ & $0.046$ & $0.11$ & $4.8\cdot 10^{-4}$ & $2.9\cdot 10^{-4}$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.53 \\
\midrule
$\mathcal{L}_{\mathrm{fwd}}^{(T)}$ & $R_{\mathrm{orth}}$ & pop. & $1$ & $4.2\cdot 10^{-5}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $100$ & $1$ & $1.9\cdot 10^{-4}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $500$ & $1$ & $2.3\cdot 10^{-4}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $1000$ & $1$ & $2.0\cdot 10^{-4}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $R_{\mathrm{vr}}$, $\mathsf{N}(0,I)$ & pop. & $1$ & $6.2\cdot 10^{-5}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $R_{\mathrm{sr}}$, $\mathsf{N}(0,I)$ & pop. & $1$ & $5.6\cdot 10^{-5}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $R_{\mathrm{vr}}$, traj. & pop. & $3.1$ & $3.7\cdot 10^{-4}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $100$ & $7.1$ & $1.7\cdot 10^{-3}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $500$ & $5.2$ & $7.5\cdot 10^{-4}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $1000$ & $5.7$ & $1.0\cdot 10^{-3}$ & -- & -- & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $R_{\mathrm{sr}}$, traj. & pop. & $7.4\cdot 10^{-4}$ & $0.068$ & $0.012$ & $2.5\cdot 10^{-3}$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  & $100$ & $6.9\cdot 10^{-4}$ & $1.2$ & $0.044$ & $0.023$ & 0.40 & 0.40 & 0.40 & 0.40 & 0.40 & 0.40 & 0.40 \\
 &  & $500$ & $1.1\cdot 10^{-3}$ & $0.91$ & $0.017$ & $0.019$ & 0.60 & 0.60 & 0.55 & 0.40 & 0.40 & 0.20 & 0.20 \\
 &  & $1000$ & $1.3\cdot 10^{-3}$ & $1.1$ & $0.028$ & $7.4\cdot 10^{-3}$ & 0.40 & 0.40 & 0.40 & 0.40 & 0.40 & 0.20 & 0.20 \\


==> tables/nonlinear_conjugacy.tex <==
$0.01$ & $10$ & $0.17$ & $0$ & linear & 0/5 & $1$ & $1$ & $0.026$ & -- & -- & 0/5 \\
 &  &  &  & MLP & 4/5 & $0.094$ & $0.99$ & $2$ & $0.11$ & $0.012$ & 4/5 \\
 & $20$ & $2.3$ & $0$ & linear & 5/5 & $0.015$ & $1$ & $0.037$ & $5.9\cdot 10^{-3}$ & $1.1\cdot 10^{-3}$ & 5/5 \\
 &  &  &  & MLP & 5/5 & $0.019$ & $0.99$ & $2$ & $0.059$ & $2.9\cdot 10^{-3}$ & 5/5 \\
 & $40$ & $54$ & $47$ & linear & 5/5 & $0.013$ & $1.4\cdot 10^{-4}$ & $4.6$ & $0.17$ & $0.07$ & 1/5 \\
 &  &  &  & MLP & 5/5 & $0.011$ & $2.3\cdot 10^{-3}$ & $2.6$ & $0.03$ & $2.2\cdot 10^{-3}$ & 5/5 \\
\midrule
$0.03$ & $10$ & $1.5$ & $0$ & linear & 0/5 & $1$ & $0.99$ & $0.21$ & -- & -- & 0/5 \\
 &  &  &  & MLP & 4/5 & $0.09$ & $0.99$ & $1.9$ & $0.12$ & $9.9\cdot 10^{-3}$ & 4/5 \\
 & $20$ & $12$ & $1$ & linear & 5/5 & $0.019$ & $1$ & $0.062$ & $0.015$ & $2.8\cdot 10^{-3}$ & 5/5 \\
 &  &  &  & MLP & 5/5 & $0.018$ & $0.99$ & $2$ & $0.054$ & $1.2\cdot 10^{-3}$ & 5/5 \\
 & $40$ & $92$ & $81$ & linear & 5/5 & $0.031$ & $8.3\cdot 10^{-4}$ & $4$ & $0.24$ & $0.088$ & 1/5 \\
 &  &  &  & MLP & 5/5 & $6.8\cdot 10^{-3}$ & $0.86$ & $1.7$ & $0.032$ & $9.3\cdot 10^{-4}$ & 5/5 \\
\midrule
$0.1$ & $10$ & $13$ & $1$ & linear & 0/5 & $0.99$ & $0.79$ & $1.2$ & -- & -- & 0/5 \\
 &  &  &  & MLP & 2/5 & $0.99$ & $0.97$ & $2.3$ & $0.14$ & $0.016$ & 1/5 \\
 & $20$ & $39$ & $41$ & linear & 5/5 & $0.051$ & $0.88$ & $0.38$ & $0.088$ & $9.0\cdot 10^{-3}$ & 1/5 \\
 &  &  &  & MLP & 5/5 & $0.02$ & $0.99$ & $1.9$ & $0.062$ & $1.6\cdot 10^{-3}$ & 5/5 \\
 & $40$ & $101$ & $94$ & linear & 5/5 & $0.061$ & $0.92$ & $0.35$ & $0.16$ & $0.013$ & 1/5 \\
 &  &  &  & MLP & 5/5 & $0.011$ & $0.98$ & $2.1$ & $0.039$ & $2.4\cdot 10^{-3}$ & 5/5 \\


==> tables/nonlinear_eps_tips.tex <==
$0.01$ & $10$ & MLP, $u = KE(x)$ & 0.65 & 0.60 & 0.50 & 0.40 & 0.38 & 0.20 & 0.20 \\
 &  & MLP, $u = KJ_E(0)x$ & 0.70 & 0.70 & 0.70 & 0.75 & 0.78 & 0.80 & 0.80 \\
 &  & linear, $u = KEx$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $20$ & MLP, $u = KE(x)$ & 1.00 & 1.00 & 1.00 & 1.00 & 0.78 & 0.25 & 0.25 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & $40$ & MLP, $u = KE(x)$ & 1.00 & 0.75 & 0.55 & 0.55 & 0.60 & 0.60 & 0.62 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\
\midrule
$0.03$ & $10$ & MLP, $u = KE(x)$ & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 \\
 &  & MLP, $u = KJ_E(0)x$ & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 & 0.80 \\
 &  & linear, $u = KEx$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $20$ & MLP, $u = KE(x)$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & $40$ & MLP, $u = KE(x)$ & 1.00 & 1.00 & 1.00 & 0.95 & 0.90 & 0.88 & 0.80 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\
\midrule
$0.1$ & $10$ & MLP, $u = KE(x)$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\
 &  & MLP, $u = KJ_E(0)x$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\
 &  & linear, $u = KEx$ & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 & $20$ & MLP, $u = KE(x)$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\
 & $40$ & MLP, $u = KE(x)$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & MLP, $u = KJ_E(0)x$ & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 &  & linear, $u = KEx$ & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 & 0.20 \\

